Learning a Diffusion Prior for NeRFs

Neural Radiance Fields (NeRFs) have emerged as a powerful neural 3D representation for objects and scenes derived from 2D data. Generating NeRFs, however, remains difficult in many scenarios. For instance, training a NeRF with only a small number of views as supervision remains challenging since it is an under-constrained problem. In such settings, it calls for some inductive prior to filter out bad local minima. One way to introduce such inductive priors is to learn a generative model for NeRFs modeling a certain class of scenes. In this paper, we propose to use a diffusion model to generate NeRFs encoded on a regularized grid. We show that our model can sample realistic NeRFs, while at the same time allowing conditional generations, given a certain observation as guidance.

==> cvpr/cvl_shortcuts.tex <==
% This is roughly version 1.1 of vcl-shortcuts, circa Dec 2016.
% Put together by Vladlen Koltun


%Set up nice tables using the tabular package
%Make \toprule and \bottomrule thicker than \midrule
\setlength\heavyrulewidth{0.10em}
\setlength\lightrulewidth{0.05em}
\setlength\cmidrulewidth{0.03em}
\newcommand{\ra}[1]{\renewcommand{\arraystretch}{#1}}

%Set up the siunitx package, particularly for using the S column type in tables
\usepackage[super]{nth}
\usepackage{nicefrac}
\sisetup{detect-weight=true,detect-inline-weight=math}
\sisetup{quotient-mode = fraction}
\sisetup{fraction-function = \nicefrac}
\robustify\bfseries


%Known issue: the following shortcuts override \gg, \ll\, and \tt, which are existing LaTeX commands. Use \ggreater and \llesser, defined below, instead of \gg and \ll. Use \texttt{} instead of \tt.
%Also \ss is taken and in some environments cannot be overridden. Use \sss for a bold `s' instead.
\def\aa{\mathbf{a}}
\def\bb{\mathbf{b}}
\def\cc{\mathbf{c}}
\def\dd{\mathbf{d}}
\def\ee{\mathbf{e}}
\def\ff{\mathbf{f}}
\def\gg{\mathbf{g}}
\def\hh{\mathbf{h}}
\def\ii{\mathbf{i}}
\def\jj{\mathbf{j}}
\def\kk{\mathbf{k}}
\def\ll{\mathbf{l}}
\def\mm{\mathbf{m}}
\def\nn{\mathbf{n}}
\def\oo{\mathbf{o}}
\def\pp{\mathbf{p}}
\def\qq{\mathbf{q}}
\def\rr{\mathbf{r}}
\def\sss{\mathbf{s}}
\def\tt{\mathbf{t}}
\def\uu{\mathbf{u}}
\def\vv{\mathbf{v}}
\def\ww{\mathbf{w}}
\def\xx{\mathbf{x}}
\def\yy{\mathbf{y}}
\def\zz{\mathbf{z}}

\def\AA{\mathbf{A}}
\def\BB{\mathbf{B}}
\def\CC{\mathbf{C}}
\def\DD{\mathbf{D}}
\def\EE{\mathbf{E}}
\def\FF{\mathbf{F}}
\def\GG{\mathbf{G}}
\def\HH{\mathbf{H}}
\def\II{\mathbf{I}}
\def\JJ{\mathbf{J}}
\def\KK{\mathbf{K}}
\def\LL{\mathbf{L}}
\def\MM{\mathbf{M}}
\def\NN{\mathbf{N}}
\def\OO{\mathbf{O}}
\def\PP{\mathbf{P}}
\def\QQ{\mathbf{Q}}
\def\RR{\mathbf{R}}
\def\SS{\mathbf{S}}
\def\TT{\mathbf{T}}
\def\UU{\mathbf{U}}
\def\VV{\mathbf{V}}
\def\WW{\mathbf{W}}
\def\XX{\mathbf{X}}
\def\YY{\mathbf{Y}}
\def\ZZ{\mathbf{Z}}

\def\aA{\mathcal{A}}
\def\bB{\mathcal{B}}
\def\cC{\mathcal{C}}
\def\dD{\mathcal{D}}
\def\eE{\mathcal{E}}
\def\fF{\mathcal{F}}
\def\gG{\mathcal{G}}
\def\hH{\mathcal{H}}
\def\iI{\mathcal{I}}
\def\jJ{\mathcal{J}}
\def\kK{\mathcal{K}}
\def\lL{\mathcal{L}}
\def\mM{\mathcal{M}}
\def\nN{\mathcal{N}}
\def\oO{\mathcal{O}}
\def\pP{\mathcal{P}}
\def\qQ{\mathcal{Q}}
\def\rR{\mathcal{R}}
\def\sS{\mathcal{S}}
\def\tT{\mathcal{T}}
\def\uU{\mathcal{U}}
\def\vV{\mathcal{V}}
\def\wW{\mathcal{W}}
\def\xX{\mathcal{X}}
\def\yY{\mathcal{Y}}
\def\zZ{\mathcal{Z}}

\def\Ae{\mathbb{A}}
\def\Be{\mathbb{B}}
\def\Ce{\mathbb{C}}
\def\Le{\mathbb{L}}
\def\Ne{\mathbb{N}}
\def\Pe{\mathbb{P}}
\def\Qe{\mathbb{Q}}
\def\Re{\mathbb{R}}
\def\Se{\mathbb{S}}
\def\Te{\mathbb{T}}
\def\Xe{\mathbb{X}}
\def\Ye{\mathbb{Y}}
\def\Ze{\mathbb{Z}}

\def\btheta{{\bm\theta}}
\def\bzeta{{\bm\zeta}}
\def\bmu{{\bm\mu}}
\def\bZero{\mathbf{0}}
\def\bOne{\mathbf{1}}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\minimize}{minimize}
\DeclareMathOperator*{\maximize}{minimize}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\trace}{tr}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\diam}{diam}

\def\eps{\varepsilon}
\def\vphi{\varphi}
\def\vsigma{\varsigma}

\def\trans{^{\top}}
\def\deg{^{\circ}}

\def\th{^{\textnormal{th}}}
\def\st{^{\textnormal{st}}}
\def\nd{^{\textnormal{nd}}}

%\ggreater and \llesser replace \gg and \ll, which have been overridden
\newcommand\ggreater{\mathbin{>\!\!\!>}}
\newcommand\llesser{\mathbin{<\!\!\!<}}

%Checkmark and cross symbols for tables
\newcommand{\YesV}{\ding{51}}%
\newcommand{\NoX}{\ding{55}}%

%Use @ instead of , in long numbers in math mode. For example, use $10@000$ rather than $10,000$.
\DeclareMathSymbol{@}{\mathord}{letters}{"3B}

\newcommand\paren[1]{\left(#1\right)}
\newcommand\abs[1]{\left\lvert#1\right\rvert}
\newcommand\norm[1]{\left\lVert#1\right\rVert}
\newcommand\tuple[1]{\left\langle#1\right\rangle}
\newcommand\inner[2]{\langle #1, #2 \rangle}

%Use \timess instead of \times in the main lines of equations, but not in superscripts or subscripts. Use the regular \times in superscripts or subscripts.
\newcommand\timess{\mathbin{\!\times\!}}

%Known issue: \nicebar is not nice in PNAS format, use \bar if submitting to PNAS.
\newcommand\nicebar[1]{\mkern 4mu\overline{\mkern-4mu#1}}

%Replace ``\yourname" and ``Name" with your name
\newcommand\yourname[1]{\textcolor{blue}{Name says: #1}}
\newcommand\vladlen[1]{\textcolor{blue}{Vladlen says: #1}}

%Paragraph heading with customizable vertical spacing. Modify the length inside \vspace to expand or contract the vertical offset preceding a new paragraph heading.
\newcommand\mypara[1]{\vspace{1mm}\noindent\textbf{#1}}

%Orient text vertically. Useful for tables and figures.
\def\rot#1{\rotatebox{90}{#1}}

%I use the self-indulgent \LaTeX operator mostly to illustrate an issue and a useful trick. The issue is that LaTeX operators eat the space that follows them, so if they occur in the middle of a sentence they eliminate the space separating the following word. But you can't just insert a space will-nilly (e.g., \LaTeX\ or \LaTeX~) because if the operator is followed by a punctuation mark then there shouldn't be a space. One solution is to write \LaTeX{}, which does the right thing but is easy to forget. The alternative, demonstrated here, is to define an operator with a name that ends with the forward slash. This also does the right thing and looks sufficiently distinctive to be memorable.
\def\latex/{\LaTeX}
\def\bibtex/{\hologo{BibTeX}}

%Miscellaneous \latex/ tips:
% To create an invisible character, use the \phantom command or its relatives: http://tex.stackexchange.com/questions/4519/how-do-i-create-an-invisible-character

% Roman numerals
\newcommand{\RN}[1]{%
  \textup{\uppercase\expandafter{\romannumeral#1}}%
}
% first fundamental form
\def\FFF{%
	\textbf{\textup{\uppercase\expandafter{\romannumeral 1}}}%
}
\def\SFF{
	\textbf{\textup{\uppercase\expandafter{\romannumeral 2}}}%
}
% First and second foundmanetal forms
% \def\FFF{\mathbf{\RN{1}}
% \def\SFF{\textbf{\RN{2}}
% \newcommand\FFF{\textup{\uppercase\expandafter{\romannumeral 1}}
% \def\FFF{\romannumeral{1}

\def\PNF{\operatorname{PNF}}

\def\oomega{\boldsymbol{\omega}}
\def\mmu{\boldsymbol{\mu}}
\def\ggamma{\boldsymbol{\gamma}}
\def\bbeta{\boldsymbol{\beta}}
\def\aalpha{\boldsymbol{\alpha}}

==> figures/architecture/architecture.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth,height=0.3\linewidth,draft=True]{example-image-a}
    \caption{\todo{architectyure}}
    \label{fig:architecture}
\end{figure*}

==> figures/edit_nerf/edit_nerf.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth,height=\linewidth,draft=True]{example-image-a}
    \caption{\todo{NeRF editing qualitative results}}
    \label{fig:edit-nerf}
\end{figure}

==> figures/teaser/teaser.tex <==
\begin{figure}[t]
  \centering
   \includegraphics[width=\linewidth,height=\linewidth,draft=True]{example-image-a}

   \caption{\todo{Teaser}}
   \label{fig:teaser}
\end{figure}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sections/drafts/abstract-metalearning.tex <==

\begin{abstract}
Recently, neural fields have been raised as an powerful signal representation.
The common paradigm to obtain a neural field representation is to conduct test-time optimization by updating the neural fields parameters according to reconstruction loss of the signal.
Such test-time optimizations, however, usually requires many iterations (thus slow), and relies on large amount of observation data to supervise.
Our paper tries to alleviate these issues by learning a network to predict initialization and optimization signal for test-time optimization.
However, naively applying meta-learning and generative models toward this problem is not feasible as there are usually limited amount of supervision available to train such meta-learner.
In this paper, we re-formulate this into learning a latent diffusion model which contains a encoder to predict the initialization and a denoiser to predict test-time optimization gradients.
We proposed a novel training objective for latent diffusion model to allow it to leverage supervision with noisy or partial observation.
% \todo{Result sentence.}
\end{abstract}

==> sections/drafts/intros-1.tex <==
\section{Introduction}\label{sec:intro}
% \todo{where do I motivate i) use of diffusion model and ii) use of}


\textbf{1. Motivation: why is it important to generate NeRFs (i.e. learning a prior over NeRF)}
%     1.1 nerf is a very good 3D representation
%     1.2 it works well when nums of views are enough
%     1.3 but it's not always the case
%     1.4 as a results it's beneficial to have prior (when there is not enough supervision)
%     - (TODO) maybe even motivate that we need 3D prior
\todo{why we care about NeRF.} NeRF  has been emerged to be a popular scene representation thanks to \todo{(advantages)} their ability to represent scenes in high fidelity.
\todo{NeRF works well there are enough views}. Generating NeRF usually requires running a test-time optimization procedure supervised with a photometric loss for a set of posed images.
\todo{issue: hard to work with few views}
This test-time optimization procedure usually requires a large number of posed images as supservision.
Without enough supervision, such optimization usually lead to bad-performance as there are multiple instantiation of NeRF with infeasible geometry that can explain well the posed image.
\todo{we need to encode priors to resolve this.}
To resolve this issue, it's essential to encode inductive prior in this test-time optimization procedure to filter out invalid representation.
\todo{what does it mean by a successful/suitable prior?}
An good inductive prior should i) works naturally well with test-time optimization regardless of the amount of supervision; ii) allow exploring all feasible solutions.


\textbf{How do people encode NeRF prior? Why are they not enough (philosophically)? Why is diffusion prior a good choice?}
% 2.1 Heuristic base: RegNeRF, RefNeRF; \todo{why are they not good enough?}
%     - Praise that this works
%     - 
% 2.2 Learning based: \todo{why are they not enough?}
%     \todo{- Check papers: VAENeRF, PixelNeRF, CodeNeRF}
%     - Encoder: directly take signal to NeRF (PixelNeRF) 
%         - restricted to specific application (e.g. image to NeRF), need to swap when the application changed (e.g. editing NeRF?)
%         - 
%     - Decoder: ? ? have people done it ?? 
% 2.3 I want to land at learning a prior for NeRF is still an interesting and unsolved question.
There are two major category of inductive prior previous research have studied.
\todo{1. heuristic prior} The first type is the heuristic to design loss function to regularize the optimization procedure~\cite{RegNeRF}. 
These heuristics tend to be applicable to many general objects, but it usually cannot complete the whole scene \todo{?short-coming of heuristic prior?}.
Alternatively, many works have explore data-generated 
\todo{learned initialization.} Prior works also have explored learning based prior by learning an initialization for the optimization procedure.
But this doesn't guarantee the the output 
\todo{discriminative-prior} \cite{PixelNeRF} - 
\todo{generative prior.}
3. Generative prior.
3.1 Using GAN \cite{EG3D, EpiGRAF} - non-trivial to inverse, so hard to use it for test-time optimization
3.2 VAE/D \cite{VAE-NeRF, CodeNeRF} - the added complexity of prior is not part of the inference; less compact; ours are faster during rendering applications.

        
\textbf{Challenge of doing generative priors with diffusion on NeRF?}
3.1 \textit{Choosing the representation is difficult.} MLP are expressive but unstructured and noncompact, hard to obtain in large scsale; global latent code has limited expressivity (due to encoder/decoder architecture). the happy medium seems to be spatial latent code - which has several advantages (i) it's easy to train (e.g. 2 minutes per ReLUF); (ii)
3.2 \textit{Test-time optimization.} Most downstream application of NeRF requires test-time optimization, so we need to choose a generative model that can organically intergrate it.
3.3 \textit{Visibility issue.} The volume rendering formulation of NeRF means that some spatial location does not 

4. How do we solve it?
4.1 Diffusion model prior on ReLUF / Plenoxels.
4.2 

==> sections/drafts/intros-2.tex <==
\section{Introduction}\label{sec:intro}

% 1. Motivation: NeRF is important, and we want to solve two problems with NeRF: generation and few-view reconstruction.
\guandao{(why we care about NeRF.)} 
NeRF  has been emerged to be a popular scene representation. 
Thanks to their ability to represent scenes in high fidelity, there have been plenty of research and application about NeRF~\todo{cite}.
% \todo{NeRF works well there are enough views}. Generating NeRF usually requires running a test-time optimization procedure supervised with a photometric loss for a set of posed images.
% \todo{issue: hard to work with few views}
\guandao{(cond. generating nerfs is difficult)}
Despite such popularity, generating NeRFs remains non-trivial for many scenarios.
For example, a common way to obtain NeRFs is through running test-time optimization with a large set of posed images as supervision.
Without enough supervision, such optimization usually lead to bad solution due to the fact that there are many possible but bad ways to explain the limited supervision.
\input{figures/teaser/teaser}

\guandao{uncond gen is difficult and not applicable to test-time-opt.}
% Learning a generative model that can generate NeRF of a particular category is also remains challenging.
Such problem can potentially be addressed by learning a generative model that can model the distribution of NeRFs.
% Most existing works learning generative models for NeRFs focus on unconditional generation tasks only, which makes many of methods difficult to apply to resolve such issue.
Many works apply variational objective (i.e. VAE, VAD)~\cite{NeRFVAE} to generate NeRFs.
Due to \todo{the limited capacity of VAE}, these works usually report results with lower resolution.
The most successful NeRF generative models usually apply GAN~\cite{EG3D,GRAF,EpiGRAF,...} to generate NeRF.
While these GAN-base methods can lead to generation of high-quality images, they usually lack of results in incorporating the learned prior in test-time optimization procedure, partially due to the difficult to inverse GAN decoder.
This makes it unclear how to incoroprate this into test-time optimization pipeline.
% Despite current progress in learning generative model for NeRFs, most existing methods focus on sampling quality of unconditional generation of NeRF representaiton, yet neglect the generative model's ability to incoroprate with test-time optimization.
% Another example is that despite the success of generative models in many modality like 2D images and 3D shapes, learning generative models for NeRF remains a very challenge problem.
\guandao{(Set-up stage: generative model for NeRF for both cond and uncond)}
This lead to the question, is it possible to design a NeRF generative model that both can  generate high-quality unconditional samples but also incorporate with test-time optimization to perform conditional generation?


\guandao{Key-insight: diffusion model can do it.}
In this paper, we propose to achieve this goal by learning a diffusion model~\cite{theoldpaper,DDPM,ScoreSDE} to generate voxel-based NeRFs.
% \guandao{0. brief intro to diff. model}
% Diffusion model is ...
\guandao{1. DFM can produce good sample}
Diffusion model has shown to have the capability to generate state-of-the-arts sampling quality (in images and videos~\cite{}).
\guandao{2. DFM can incorporate to test-time opt.}
The sampling procedure of diffusion model is iterative.
This suggests that one can parallel the sampling procedure with test-time optimization by using test-time optimization loss as guidence for the sampling procedure.
This suggests that diffusion model can be a good solution to both generate high-quality NeRFs and support test-time optimization with few-views.

\guandao{Technical challenges: 1. representation; 2. things like}
Learning a diffusion model for NeRF, however, is non-trivial.
First, we need to find a NeRF representation where diffusion model can work.
Since diffusion model usually works well in a grid-structure representation, we propose to represent NeRFs in the form of ReLU fields~\cite{ReLU-F}.
% ReLU fields are fast to train and it has many advantages as it is in the grid structure and it's also easy to preprocess and generate.
Second, learning diffusion in ReLU fields is challenging since the diemsnions have different distribution.
The dimension that contains radiance density has drastically different distribution from the dimension that contains radiance information.
To tackle this, we propose a \textbf{novel diffusion architecture} that contains separate denoiser and noise scheduler for the radiance and density channels.
\todo{Third, denoising radiance information is difficult because most of 3D location the radiance are invisible.
To address that we propose a novel radiance denoiser that can reason about geometry based on the output the denoiser by computing the visibility field of the current ReLU field.
}
\guandao{hightlight the results}
\todo{We show that our model is able to achieve SOTA results in few-view NeRF reconstruction and generation in SRN dataset}.

To summarize, the main contributions of our works are:
\begin{enumerate}
    \item We propose a novel diffusion model architecture that allows generation of NeRF representing in the form of ReLU fields.
    \item We propose a method to train diffusion model with data where different channels have drastically different distributions.
    \item \todo{}
\end{enumerate}







==> sections/drafts/intros-draft-2.tex <==
\textbf{1. Motivate: Learn a generative model for NeRF?}
- generate NeRfs
- use it for guide test-tiem optimization 
    - single-view neRF
    - editing ....

\textbf{2. How does prior learn generative for NeRF? Why is it not enough?}
% - Normalization flows (no one has tried it)
% - Auto-regressive (no one has tried it, try different)
- GAN ~\cite{EG3D,EpiGRAF} GAN is hard to inverse, so it's not clear how to incorporate this GAN prior in test-time optimization.
- VAE ~\cite{NeRF-VAE} quality is bad
- Diffusion model
    - easy to use for test-time optimization
    - high quality


==> sections/drafts/intros-draft-3.tex <==
\section{Introduction}
1. Diffusion is cool.
2. Mostly success in 2D images
3. NeRF is very important domain
4. Can we apply diffusion to NeRF? - will be
5. 

==> sections/drafts/intros-metalearning.tex <==
\section{Introduction}


% 1. Motivation
% - (Nueral fields) Neural field is useful
% - (Test-time optimization) Common paradigm of fitting neural field is using test-time optimization
%     - (Advantage) More generalize
%     - (Adaptability) Can adapt to different data
% - (Prob. of test-time optimization) start from scratch
%     - takes long to converge
%     - requires a lots of supervision
% - (motivate the goal) learning a prior for test-time optimization
%     - people have already trained it several times
%     - wouldn't it be nice that one can learn from previous training experiences to accelerate the test-time optimization?

Neural fields are neural networks that transform spatial coordinates to signals~\todo{\cite{}}.
Neural fields has raised as a powerful representation for many types of signals including images~\todo{\cite{}}, signed distance functions~\todo{\cite{}}, and radiance fields~\todo{\cite{}}.
A common paradigm to obtain a neural fields is to conduct \textit{test-time optimization}.
Specifically, one would run gradient-based optimization on reconstruction loss between the test data and the synthesis results from a random initialization of the neural fields parameters until the reconstruction loss converges \todo{Will recon loss perspective too narrow?}.
% ~\todo{(a concise-way to describe test-time optimization, show that there are two components: initialization and gradient-based updates}.
Such test-time optimization schema has shown to be very robust to different instance of signals ~\todo{\cite{}} and .. \todo{advantages of test-time optimization}.
However, test-time optimization can takes lots of steps to converge~\todo{\cite{INstance-NGP}}.
It can lead to bad results when the gradients are not reliable due to lack of test-time observation~\todo{\cite{RefNeRF}}.
One reason for these issues is that the test-time optimization is ran independently from scratch every time.
It makes it difficult to leverage prior knowledge (potentially learned from large amount of data) to accelerate test-time optimization or reduce the supervision required.
% For example, even if one has perform test-time optimization for a thousand times in the past, there is very little tool that can transfer 
Is it possible to a method that can learn from prior data how to better perform test-time optimization on neural fields?

% GOAL:
% v0: Learning a prior for test-time optimization of neural fields with
%     i) partial supervision
%     ii) mixed supervision
% v1: learn prior knowledge for neural fields

% 2. Why is it not solved yet? - there are two challenges




% 3. Our method: 
%     - learn more than the initialization.
%     - learn it without roll-out using diffusion model.
%     - allow leveraged of mixed supervision.
In this paper, we proposed a novel way to learn the initializer and optimizer for performing test-time optimization of neural fields.
There are three components of our model.
The initializer that takes data and predicts an initialization of the latent code which parameterized the signals; the neural fields decoder that outputs the signal; and an latent diffusion model that refines the latent code.
Different from existing latent diffusion models~\cite{LDM-1, LDM-2, VDM, LSGM} which ask the encoder to predict the latent code corresponding to the clean image, we relax this assumption to allow the encoder to predict a noisy latent code.
This changes allow the decoder to work with both fully observed signal and partially observed signals.


    


    

% v0:
%     - Say that there are several ways to learn the prior for test-time optimization
%     - Initialization
%     - Optimization
%     - Final output (if we can motivate


    


\ignore{
Writing links:
\url{https://github.com/jbhuang0604/awesome-tips#writing}
\url{https://billf.mit.edu/sites/default/files/documents/cvprPapers.pdf}

TOM gives an overview:
Need to include:
1. Setting up the goal and the motivation. (e.g. a sentence: what's the goal of our project)
    - this should encore in the related work and the experiment
    In my case: is it
    a) enable mix supervision?
    b) sparse observation?
    c) learning prior for test-time optimization?
    Can start with the goal and then?
2. Summary of related works (why is it hard, why is it not achieved before)
    - there is no method that achieve this goal now
    - setting up the fundamental problem 
3. Approach - hitting the fundamental problem 
    - justification why it should work 
    - optionally add a little bit of details of what's interesting about the approach (e.g. what I called the technical challenge)
    - summary of the results (hightlight the results)

Optionally: adding the contribution bullet points (more for reviewers)
- contributions are :
i) nouns 
ii) think of it as claims we verify in the paper/experiments
}

\ignore{
% 2. Why is it not solved yet? - there are couple challenges
%     i) hyper-network: directly predicting the weights/parameterizatio of the neural fields
%     ii) learning initialization provides very little prior
%     iii) learning to predict gradient requires roll-out, hard to train
% TODO: where to position DeepSDF?
%     iv) applying generative model/diffusion model - requires full observation, which isn't always the case.
Prior works have approached this problem mainly in three ways.
One way is to formulate this problem as a meta-learning problem. Applying deep meta-learning algorithms such as MAML~\cite{MAML} and Reptile~\cite{Reptile} to this problem has shown to be effective in reducing the number of optimization steps~\todo{~\cite{MetaSDF, LearnInit, PlenopticNF}}.
But these meta-learning algorithms usually need to back-prop through a series of roll-outed optimization steps, making them difficult to scale.
Another approach is to train hyper-network to directly predicting the parameterization of the neural fields ~\todo{\cite{SIREN, TransitINR}}, then apply test-time optimization on the predicted neural fields.
These approaches are easier to train as it avoid the backpropogating through the rollout steps.
But it faces challenges when the test-time data is limited, when the network is asked to generalize to test-time signals.
The third class of methods approach this problem by learning a generative model of the parameterization of neural fields.
Training a generative model, however, requires a large amount of well-observed signals.
Such data is usually not available in real-world scenario.
\todo{it's not clear what's the foundamental problem right here - is it rollout? is it lack of training time supervision?}
\todo{Learned initilization: one per category; hypernetwork : one per instance}
}

==> sections/drafts/methods.tex <==
\section{Methods}\label{sec:method}

\guandao{Set-up the stage of our method.}
% \guandao{1. restate the purpose: we want to have a generative prior that's capable of doing test-time optimization}
Recall from Sec~\ref{sec:intro}, our goal is to build a generative prior for NeRFs that's capable of not only generate NeRFs unconditionally, but also is capable of being used for different test-time optimization algorithms.
One good way to achieve it is to use diffusion model to learn the generative prior for NeRF since diffusion model has the capacity to incorporate different guidance.
To train a diffusion prior for NeRFs, however, is non-trivial because of several reasons.
\todo{Life can be easier if I motivate to learn diffusion model for ReLU-F (instead of NeRF in general).}
First, it's not clear what's the best ways to represent NeRF so that the diffusion generative model is able to denoise it prorgessively.
Second, it's also not clear what's the right network architecture that can denoise NeRFs.

In this section, we will tackle these challenges one-by-one.
We follow~\cite{latent-diffusion, PointFlow, ShapeGF} to break down the generation procedure in two stages: first stage will learn a latent representation of the scene and the second stage will learn a generative model in that latent representation.
In our first stage, we propose to train regularized ReLU-field, a representation of NeRF that's suitable to learn a diffusion model.We will show that regularized ReLU fields are are easy to obtain and they can be denoised using standard U-Net architecture since it's represented in a grid (Sec~\ref{sec:first-stage}).
In our second stage, we will train a DDPM model on the regularized ReLU-fields. 
Specifically, we propose a novel double-UNet architecture and diffusion loss that's able to account for the drastically different statistic properties between the density and the albedos (Sec~\ref{sec:second-stage}).
Finally, we propose a way to use reconstruction guidance~\cite{video-diffusion} to perform test-time optimization for a variety of 3D tasks including single-view NeRF reconstruction and image-guided editing (Sec~\ref{sec:test-time-opt}).

\subsection{Regularized ReLU-F}\label{sec:first-stage}
\input{figures/first_stage/first_stage}
\todo{Maybe make this more generalize? leave open choice for other representation, but say that we will focus on this representation for this exploration.}

\guandao{argue why we want ReLU-F}
To learn a diffusion generative prior for NeRF, it's essential to find the right representation of NeRFs that's suitable to be learned by diffusion model.
A good representation should have the following properties:
a) \textit{accessible}. training a diffusion model requires a lots of data, so we need our representation to be easy to obtain
b) \textit{structured}. In order for diffusion model to be able to denoise it progressively, we need the model to have structure, and
c) \textit{expressive}. Since we want to be able to represent signals in high fedelity.
Naively representing NeRF with MLP (weights) doesn't work since it's not fast enough to train.
Latent code modulated MLP is hard to train (since it needs to propogate gradient across machine) and it's usually limited in expressivity.
Spatially modulated latent grid is also difficult to train since it requires gradient syncing across machines.
With these considerations, we believed that the best candidate is to represent it with ReLu fields because it's fast to train (takes about 2 minutes per scene), expressive, and it has a spatial structure.
With this said, our first stage will try to obtain NeRFs in the form of ReLu fields.

Specifically, we assume we have a dataset of $N$ scenes, each of which has $M$ posed images: $\{(\rvp_{ij}, I_{ij})\}_{j=1}^M\}_{i=1}^N$, where $\rvp_{ij}$ is the $j^{th}$ camera posed and pixel images for the $i^{th}$ scene.
For each scene $i$, we want to train a ReLU field using the posed images $\{(\rvp_{ij}, I_{ij})\}_{j=1}^N$.
A ReLU-field $F_\rmV:\sR^{3}\times \sR^2 \mapsto \sR \times \sR^3$, which takes a tuple of 3D coordinate and direction and output a tuple of density and RGB value.
$F_\rmV$ is parameterized by a grid of size $\rmV \in \sR^{R\times R \times R \times 4}$. \todo{not necessarily 4, it's 1 for density then d for whatever needed for the color}: $F_\rmV(\rvx, \rvd) = f(\operatorname{interp}(\rmV, \rvx), \rvx, \rvd)$, where $\operatorname{interp}$ is trilinear interpolation.
The function $f$ is parameter-less that takes the $4$-D interpolated feature to predict the final density and RGB value. 
The density is defined as $f(\rvv, \rvx, \rvd)_{den} = \exp(\alpha\rvv[0] + \beta)$ and the RGB color is obtained by $f(\rvv, \rvx, \rvd)_{rgb} = \operatorname{Sigmoid}(\rvv[1:4])$.
\todo{We ignore position and view direction here}.

The parameter $\rmV$ is optimized by loss objective showed in Equation~\ref{eq:NeRF-color}.
But naively optimizing this objective without any regularization will lead to an ill-posed problem as there are many different ways to instantiate the density and the color field to satisfied the photometric loss.
This is due to the fact that there are many voxels in the field that is either 1) \textit{free-space} (i.e. having very low density value), and/or 2) \textit{occluded} (i.e. there is no ray that can create substantial alpha composition value for the color at that location).
Letting these invisible voxels to be set into arbitrary value does not affect the final rendered image, but it makes the data set more complex and less easy to be denoised.
As shown in Figure~\ref{fig:first-stage}.
To alleviate this issue, we regularize these fields with the following two losses:

\paragraph{Density sparsity regularization.} We encourage the field to have sparse density, so that it only put high density in the places where the color does matters:
\begin{align}
    \Ls_{d}(\rmV) = \norm{\rmV[..., 0] - d_{min}}_1,
\end{align}
where $d_{min}$ denotes a hyper-parameter of pre-activation minimal density. 
We set it such that $\exp(d_{min}\alpha + \beta) \approx 0$.

\paragraph{Color constancy regularization.} We encourage the color of the field to be as white as possible by putting a huber-loss between the voxel color to a white color:
\begin{align}
    \Ls_{c}(\rmV) = \begin{cases}
        \frac{1}{2}\norm{\rmV[..., 1:4] - c}_2 &\text{if } \abs{\rmV[..., 1:4]} < \delta \\
        \delta\paren{\abs{\rmV[..., 1:4] - c} - \frac{1}{2}\delta}\ & \text{otherwise}
    \end{cases},
\end{align}
where $c$ is the default color we want the albedo volume to have.
Currently we set it to color white.

Finally, our regularized ReLU-Fields are training with combining three losses:
\begin{align}
    \Ls_d(\rmV) + \Ls_c(\rmV) + \sum_{j=1}^M \Ls_{NeRF}(\rmV, \rvp_{ij}, I_{ij}).
\end{align}
Figure~\ref{fig:first-stage} shows that with these regularization, we are able to obtain fields with more structured without sacrificing the quality and convergence speed (about 2 minutes). \todo{in the figure, show PSNR and time}


\input{figures/architecture/architecture}
\subsection{Learning a Diffusion Prior in NeRF}\label{sec:second-stage}

The previous section has given us a set of NeRFs, parameterized by $\{\rmV_i\}_{i=0}^N$, where $f_{\rmV_i}$ is the radiance field for scene $i$.
We would like to learn a diffusion model $p_\theta(\rmV)$ to model the distribution of $q(\rmV)$, which we assumed $\rmV_i$ are sampled from.
Naively applying diffuion model on this dataset, however, leads to bad performance due to following reasons.
First, the distribution of density is drastically different from the distribution of colors, this makes it difficult to find a common noise schedule $\alpha_t$ and $\sigma_t$ that can work for both the densty and color dimension.
Second, RGB in the visible places plays much more important role than RGB value in the free or occluded voxels; which suggests that we need to encode into the diffusion architecture and loss the idea of visibility in order to make sure it has enough capacity to denoise properly.
Toward these ends, we design a novel diffusion model architecture and objectives.

\paragraph{Separate Noise Schdule.} 
Since the distribution of density is drastically different from the distirbution of color, it makes sense to add noise to these two distribution separately.
Toward this end, we define two separate noise schedule, one for density and the other for the RGB field:
\begin{align}
    q(\rmD_t|\rmV) &= \gN(\alpha_t^{(d)}\rmV[..., 0], \sigma_t^{(d)}\rmI) \\
    q(\rmC_t|\rmV) &= \gN(\alpha_t^{(c)}\rmV[..., 1:4], \sigma_t^{(c)}\rmI),
\end{align}
where $\rmD_t \in \sR^{R\times R\times R}$ and $\rmC \in \sR^{R\times R\times R \times 3}$, and $t\in [0, 1]$.
Let $\rmV_t = \operatorname{Concat}[\rmD_t, \rmC_t]$.
\todo{Show that add noise to density affects more visual than adding noise the RGB?}
With this definition, the diffusion generative model can be written as :
\begin{align}
    p_\theta(\rmV) = \int_{\rmV_:}p(\rmV_1)\prod_{i=1}^T p_\theta(\rmV_{s(i)} | \rmV_{t(i)})d\rmV_:
\end{align}.

\paragraph{Double U-Nets.}
We need to build an architecture that's capable of modeling the distribution $p_\theta(\rmV_{s(i)} | \rmV_{t(i)})$, which denoise the representation $\rmV_{t(i)}$.
\todo{I think we still need the motivation here - it's not clear why the original UNet wouldn't work}.
In order to denoise the field, it's essential for the network to encoded prior knowledge about geometry and visibility. 
Naively training a single U-Net makes it difficult to encode such prior knowledge, which in parts cause the need of training a very large model for a very long time.
We propose to instead encode such information explicitly in the architecture by proposing a double U-Net : one to denoise the density and the other to denoise the color given the denoised density.

Specifically, we first parameterize $p_\theta(\rmD_{s(i)} | \rmV_{t(i)})$ using a U-Net $D_\theta$ that takes noise level $t$ and the noisy density and return the clean density:
\begin{align}
\hat{\rmD}_{s(i)} &= D_\theta\paren{\rmD_{t(i)}, t(i)} \\
p_\theta\paren{\rmD_{s(i)}|\rmV_{t(i)}} &= \gN(\alpha_t^{(d)}\hat{\rmD}_{s(i)} , (\sigma_t^{(d)})^2\rmI).
\end{align}
The second U-Net $C_\theta$ will then denoise the color volume taking the noise level $t(i)$, the noisy color $\rmC_{t(i)}$, and also the output of $D_\theta$ (i.e. the estimated clean density) as inputs:
\begin{align}
\hat{\rmC}_{s(i)} &= C_\theta(\rmC_{t(i)}, , t(i)) \\
p_\theta\paren{\rmC_{s(i)}|\rmV_{t(i)}} &= \gN(
\alpha_t^{(c)} \hat{\rmC}_{s(i)}, (\sigma_t^{(c)})^2\rmI).
\end{align}
Please see Figure~\ref{fig:architecture} for an illustration of the architecture.

\paragraph{Visibility-aware Diffusion Loss.}
Finally, optimizing the ELBO of $p_\theta(\rmV)$ yields the following objective:
\begin{align}
    \Ls_{T} = \frac{T}{2}\E_{\rveps,t} \left[w_c(t)\norm{\rmC-\hat{\rmC}} + w_d(t)\norm{\rmD - \hat{\rmD}]}\right],
\end{align}
where $\rmD = \rmV[..., 0]$ and $\rmC=\rmV[..., 1:4]$ and $w_d(t)$, $w_c(t)$ are weights for density and color respectively.
However, this loss tend to penalize equally the RGB error at the region of free/occluded space comparing to the solid RGB values, yet these RGB values do not contribute much to the final rendered performance.
With this consideration, we propose a visibility aware diffusion loss to make our diffusion model focus on the solid region.
To achieve it, we replace $w_c(t)$ with $w_c(t, \rmD)$, which is defined as:
\begin{align}
    w_c(t, \rmD) = w_c(t) + \operatorname{1}(\rmD > \tau),
\end{align}
where $\tau$ is a hyperparameter threshold.





\subsection{Test-time Optimization}\label{sec:test-time-opt}
Now we've obtained a generative prior in the form of a diffusion model, so we are able to sample Relu-F volume $\rmV_0$ with ancestral sampling:
\begin{align}
    \rmV_1 \sim \gN(\vzero, I), \rmV_{s(i)} \sim p_\theta(\rmV_{s(i)} | \rmV_{t(i)}), \forall i \in [1, T].
\end{align}
As mentioned in Sec~\ref{sec:intro}, we want to build a generative prior that's also capable of doing conditional sampling.
Specifically, given a conditional observation $y$ and a function that can produce the observation $p(y|\rmV)$, we would like to sample $\rmV$ from $p_\theta(\rmV|y)$.
This can be achieved by updating the same ancestral sampling with the conditional probability:
\begin{align}
    \rmV_1 \sim \gN(\vzero, I), \rmV_{s(i)} \sim p_\theta(\rmV_{s(i)} | \rmV_{t(i)}, y), \forall i \in [1, T].
\end{align}
The conditional distribution $p_\theta(\rmV_{s(i)} | \rmV_{t(i)}, y)$ can be estimated using Bayes' Rule:
\begin{align}
    p_\theta(\rmV_{s(i)} | \rmV_{t(i)}, y) \propto p_\theta(y | \rmV_{s(i)})p_\theta(\rmV_{s(i)} | \rmV_{t(i)}),
\end{align}
as long as we are able to estimate guidance probability $p_\theta(y | \rmV_t)$.

\todo{use single-view recon as example here}.
In the application of single-view reconstruction, the observation $y$ will be an image from a given pose $\rvp$,
One way to define $p_\theta(y|\rmV_t)$ is to directly use the learning objective $\Ls_{NeRF}$.
An alternative way to define $p_\theta(y|\rmV_t)$ is to use the denoised version of the volume $\hat{\rmV}$. 
In our test-time optimization algorithm, we will use both guidance.

In summary, our conditional generation algorithm can be seen below:
\begin{algorithm}
\caption{Diffusion-Guided Test-time Optimization}\label{alg:cap}
\begin{algorithmic}
\Require $n \geq 0$
% \Ensure $y = x^n$
\State $\rmV \sim \gN(\vzero, I)$
\For{$i=1\dots T$}
\State $\rmV_{t(i)} \gets \rmV$
\State $\rmV \gets p_\theta(\rmV_{s(i)} | \rmV_{t(i)})$
\For{$j=1\dots K$}
\State $\rmV \gets \rmV + \alpha \nabla_{\rmV} \log{p_\theta(y|\rmV)}$
\EndFor
\EndFor
\end{algorithmic}
\end{algorithm}

==> tables/ablation.tex <==
% Please add the following required packages to your document preamble:
\begin{table}[t]
\centering
\caption{\todo{Ablation of first stage and diffusion model}}
\begin{tabular}{@{}llllll@{}}
\toprule
 & \multicolumn{2}{c}{Generation} & \multicolumn{3}{c}{1-View Recon} \\ 
 \cmidrule(l){2-3}\cmidrule(l){4-6} 
 & FID & KID & PSNR & SSIM & FID \\\midrule
- $\Ls_{d}$ &  &  &  &  &  \\
- $\Ls_{c} $ &  &  &  &  &  \\
- D-UNet &  &  &  &  &  \\
- VisLoss &  &  &  &  &  \\
Ours &  &  &  &  &  \\ \bottomrule
\end{tabular}
\end{table}

==> tables/few_view_recon.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{booktabs}
% \begin{table}[]
% \begin{tabular}{@{}llll@{}}
% \toprule
%           & \multicolumn{3}{c}{SRN Car (1 view)} & \multicolumn{3}{c}{SRN Chair (1 view)} \\ \cmidrule(l){2-4}\cmidrule(r){5-7} 
%           & PSNR        & SSIM      & FID        & PSNR        & SSIM       & FID         \\ \midrule
% SRN       & 22.25       & 0.88      & 41.21      & 22.78       & 0.89       & 26.51       \\
% PixelNeRF & 23.17       & 0.89      & 59.24      & 23.72       & 0.9        & 38.49       \\
% VisonNeRF & 22.88       & 0.9       & 21.31      & 24.48       & 0.92       & 10.05       \\
% CodeNeRF  & 23.8        & 0.91      & -          & 23.66       & 0.9        & -           \\
% 3DiM      & 21.01       & 0.57      & 8.99       & 17.05       & 0.53       & 6.57        \\ \midrule
% Ours      &             &           &            &             &            &             \\ \bottomrule
% \end{tabular}
% \end{table}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]
\centering
\caption{\todo{Few-view reconstruction results.
}}
\begin{tabular}{@{}llll@{}}
\toprule
          & \multicolumn{3}{c}{SRN Car (1 view)}   \\ \cmidrule(l){2-4}
          & PSNR          & SSIM       & FID       \\ \midrule
SRN       & 22.25         & 0.88       & 41.21     \\
PixelNeRF & 23.17         & 0.89       & 59.24     \\
VisionNeRF & 22.88         & 0.9        & 21.31     \\
CodeNeRF  & 23.8          & 0.91       & -         \\
3DiM      & 21.01         & 0.57       & 8.99      \\ \midrule
Ours      & $\sim$19      &            &           \\ \midrule
          & \multicolumn{3}{c}{SRN Chair (1 view)} \\ \cmidrule(l){2-4}
          & PSNR          & SSIM       & FID       \\\midrule
SRN       & 22.78         & 0.89       & 26.51     \\
PIxelNeRF & 23.72         & 0.9        & 38.49     \\
VisionNeRF & 24.48     & 0.92          & 10.05.    \\
CodeNeRF  & 23.66     & 0.9           & -          \\
3DiM      & 17.05         & 0.53          & 6.57          \\ \midrule
Ours      &               &            &           \\ \bottomrule
\end{tabular}
\end{table}

==> tables/generation.tex <==
\begin{wrapfigure}{r}{0.5\textwidth}
    % \begin{table}[t]
    \centering
    \caption{\todo{Generation results in ShapeNet cars.}}
    
    \begin{tabular}{@{}lll@{}}
    \toprule
             & FID  & KID   \\ \midrule
    GIRAFFE  & 27.3 & 1.703 \\
    PIGAN    & 17.3 & 0.932 \\
    EG3D     & 2.75 & 0.097 \\ \midrule
    Ours     & $~42$&       \\ \bottomrule
    \end{tabular}
    % \end{table}  
\end{wrapfigure}

